A Small Universal Petri Net

A universal deterministic inhibitor Petri net with 14 places, 29 transitions and 138 arcs was constructed via simulation of Neary and Woods' weakly universal Turing machine with 2 states and 4 symbols; the total time complexity is exponential in the running time of their weak machine. To simulate the blank words of the weakly universal Turing machine, a couple of dedicated transitions insert their codes when reaching edges of the working zone. To complete a chain of a given Petri net encoding to be executed by the universal Petri net, a translation of a bi-tag system into a Turing machine was constructed. The constructed Petri net is universal in the standard sense; a weaker form of universality for Petri nets was not introduced in this work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{190}
\providecommand{\publicationstatus}{T. Neary and M. Cook (Eds.):\\
Machines, Computations and Universality (MCU 2013)\\
EPTCS 128, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.128.22}{10.4204/EPTCS.128.22}}
\pdfoutput=1

